O Peer, Where Art Thou? Uncovering Remote Peering Interconnections at IXPs

Internet eXchange Points (IXPs) are Internet hubs that mainly provide the switching infrastructure to interconnect networks and exchange traffic. While the initial goal of IXPs was to bring together networks residing in the same city or country, and thus keep local traffic local, this model is gradually shifting. Many networks connect to IXPs without having physical presence at their switching infrastructure. This practice, called Remote Peering, is changing the Internet topology and economy, and has become the subject of a contentious debate within the network operators' community. However, despite the increasing attention it attracts, the understanding of the characteristics and impact of remote peering is limited. In this work, we introduce and validate a heuristic methodology for discovering remote peers at IXPs. We (i) identify critical remote peering inference challenges, (ii) infer remote peers with high accuracy (>95%) and coverage (93%) per IXP, and (iii) characterize different aspects of the remote peering ecosystem by applying our methodology to 30 large IXPs. We observe that remote peering is a significantly common practice in all the studied IXPs; for the largest IXPs, remote peers account for 40% of their member base. We also show that today, IXP growth is mainly driven by remote peering, which contributes two times more than local peering.

==> ground-truth-rtt.tex <==
\begin{figure}[t]
	\begin{center}
		\includegraphics[clip,width=0.8\columnwidth]{gt-rtt-diffs.png}
		\vspace{-1em}
	\end{center}
	\caption{ECDF of minimum RTTs for remote and local peers in the validation dataset. $18\%$ of the remote peers have RTT of less than 1ms while $40\%$ have RTT of less than $10ms$.
    }
	\label{fig:ground-truth-rtt}
    \vspace{-1.2em}
\end{figure}

==> inference-heuristic-contribution.tex <==
\begin{figure}[t]
	\begin{center}
		\includegraphics[clip,width=0.95\columnwidth]{inference-heuristic.png}
		\vspace{-1em}
	\end{center}
	\caption{Fraction of inferences contributed by each step of our algorithm for the 30 largest IXPs in our results.}
	\label{fig:inference-heuristic-contribution}
    \vspace{-1.2em}
\end{figure}



==> ixp-facilities-distance.tex <==
\begin{figure}[t]
	\begin{center}
		\includegraphics[clip,width=0.7\columnwidth]{ixp-facilities-distance.png}
		\vspace{-1em}
	\end{center}
	\caption{The maximum distance between the facilities of each IXP, compared to the number of IXP members. 
We consider IXPs with facilities over 50km apart (red line) as \textit{distributed}, which correspond to 14\% of the total IXPs and 10 of the largest 50 IXPs.}
	\label{fig:ixp-facilities-distance}
    \vspace{-1.2em}
\end{figure}

==> method-steps.tex <==
\begin{figure}[t]
	\begin{center}
\includegraphics[clip,width=0.95\columnwidth]{method-steps.png}
		\vspace{-1em}
	\end{center}
	\caption{Summary of steps of remote/local peering inference methodology (gray: data inputs, green: steps, blue: decision-nexus).}
	\label{fig:method-steps}
    \vspace{-1.2em}
\end{figure}

==> multirouter-cdf.tex <==
\begin{figure}[t]
	\begin{center}
		\includegraphics[clip,width=0.95\columnwidth]{multirouter-cdf.png}
		\vspace{-1em}
	\end{center}
	\caption{CDF of far-end IXP per near-end IP and near-end router (group of IP aliases), for the ASes that are members in more than one IXPs. Almost 90\% of the routers are interconnected to more than one IXP.}
	\label{fig:multirouter-cdf}
\end{figure}
\begin{figure}[t]
	\begin{center}
		\includegraphics[clip,width=0.95\columnwidth]{multirouter-type.png}
		\vspace{-1em}
	\end{center}
	\caption{Multirouter type per number of --next hop-- IXPs.}
	\label{fig:multirouter-type}
    \vspace{-1.2em}
\end{figure}

==> pdb_website_facilities.tex <==
\begin{figure}[t]
	\begin{center}
		\includegraphics[clip,width=0.95\columnwidth]{fig_scatter_nb_DCs_logscale.eps}
		\vspace{-1em}
	\end{center}
	\caption{IXP facility data collected from IXP websites compared to PeeringDB (PDB).}
	\label{fig:pdb_website_facilities}
    \vspace{-1.2em}
\end{figure}

==> ping-measurements.tex <==
\begin{figure}[!t]
\centering
	\subfloat[Locations of IXPs with ping vantage points.]{
		\includegraphics[clip,width=0.99\columnwidth,valign=t]{ixp_lgs.png}
		\label{fig:ixp_lgs}
	}
     \hfill 
	\subfloat[ECDF of the the minimum RTTs for each responsive IXP peering interface.]{
		\includegraphics[width=0.95\columnwidth,valign=t]{ping-rtts.png}
		\label{fig:ping-rtts}
	}
	\caption{Results of our ping measurement campaign.
    40\% of the responsive IXP interfaces have a minimum RTT of more than 1ms}
	\label{fig:ping-measurements}
    \vspace{-1.2em}
\end{figure}

==> ping-vantage-points.tex <==
\begin{figure}[t]
	\begin{center}
		\includegraphics[clip,width=0.8\columnwidth]{ixp_lgs.png}
		\vspace{-1em}
	\end{center}
	\caption{Locations of IXPs with ping vantage points.}
	\label{fig:ping-vantage-points}
    \vspace{-1.2em}
\end{figure}

==> traceroute_drtt.tex <==
\begin{figure}[t]
	\begin{center}
		\includegraphics[clip,width=0.95\columnwidth]{traceroute_rtt.png}
		\vspace{-1em}
	\end{center}
	\caption{Example of IXP crossing in a traceroute path. $IP1$ belongs to address space of the near-end AS peer, while $IP3$ belongs to the IXP address space. For each IXP crossing we calculate the RTT difference $RTT_2 - RTT_1$.}
	\label{fig:traceroute_rtt}
    \vspace{-1.2em}
\end{figure}
